Out of Distribution Detection via Neural Network Anchoring

Our goal in this paper is to exploit heteroscedastic temperature scaling as a calibration strategy for out of distribution (OOD) detection. Heteroscedasticity here refers to the fact that the optimal temperature parameter for each sample can be different, as opposed to conventional approaches that use the same value for the entire distribution. To enable this, we propose a new training strategy called anchoring that can estimate appropriate temperature values for each sample, leading to state-of-the-art OOD detection performance across several benchmarks. Using NTK theory, we show that this temperature function estimate is closely linked to the epistemic uncertainty of the classifier, which explains its behavior. In contrast to some of the best-performing OOD detection approaches, our method does not require exposure to additional outlier datasets, custom calibration objectives, or model ensembling. Through empirical studies with different OOD detection settings -- far OOD, near OOD, and semantically coherent OOD - we establish a highly effective OOD detection approach. Code to reproduce our results is available at github.com/LLNL/AMP

==> related.tex <==
%\textbf{Anchoring:}
%
\textbf{OOD Detection:} Several approaches have shown promise in detecting OOD samples using pre-trained classifiers -- from early works directly using prediction entropy \citep{guo2017calibration} as the score itself, to sophisticated approaches like ODIN \citep{odin}, energy-based optimization \citep{energyood}, Gram matrices (GM) \citep{sastry2020detecting}, OE \citep{hendrycks18oe}, Mahalanobis \citep{mahalanobis} etc. Many of these approaches rely on exposure to outliers (OOD data) to calibrate their predictions to further improve OOD performance. Some recent methods also involve \emph{post-hoc} calibration on the validation set, e.g., GM and AVuC \citep{krishnan2020improving}. In this paper, we are interested in OOD detection without access to outlier data,  and we show that \name works competitively, and often outperforms, these methods. 

\textbf{OOD with Uncertainties:} In parallel, there have been several approaches that evaluate the quality of uncertainties using OOD detection, since uncertainties are expected to be larger on OOD samples. For example, DUQ \citep{van2020uncertainty} uses a kernel distance to a set of class-specific centroids defined in the feature of a deep network as the measure for uncertainty. Another recent technique is DEUP \citep{jain2021deup} which trains an explicit epistemic uncertainty estimator for a pre-trained model. More generally, Bayesian methods \citep{neal2012bayesian} are among the most common kinds of uncertainty estimators today, but they are not easily scalable to large datasets and are known to be outperformed by model ensembling \citep{lakshminarayanan2016simple}. Monte Carlo Dropout \citep{gal2016dropout} is a scalable alternative to Bayesian methods in that it approximates the posterior distribution on the weights via dropout to estimate uncertainties. However, it is well known that dropout tends to overestimate uncertainties as it has the risk of sampling the parameter space in regions that are potentially far away from the local minima. Deep Ensembles \citep{lakshminarayanan2016simple} showed a simple way to obtain accurate uncertainties in a task-agnostic and model-agnostic fashion. Anchoring models also produce unreliability estimates in the form of prediction variance, and we compare with several different uncertainty estimators for OOD and show improved detection performance.


